Few-Shot, No Problem: Descriptive Continual Relation Extraction

Few-shot Continual Relation Extraction is a crucial challenge for enabling AI systems to identify and adapt to evolving relationships in dynamic real-world domains. Traditional memory-based approaches often overfit to limited samples, failing to reinforce old knowledge, with the scarcity of data in few-shot scenarios further exacerbating these issues by hindering effective data augmentation in the latent space. In this paper, we propose a novel retrieval-based solution, starting with a large language model to generate descriptions for each relation. From these descriptions, we introduce a bi-encoder retrieval training paradigm to enrich both sample and class representation learning. Leveraging these enhanced representations, we design a retrieval-based prediction method where each sample "retrieves" the best fitting relation via a reciprocal rank fusion score that integrates both relation description vectors and class prototypes. Extensive experiments on multiple datasets demonstrate that our method significantly advances the state-of-the-art by maintaining robust performance across sequential tasks, effectively addressing catastrophic forgetting.

==> sections/3.1.retrieval.tex <==
% \subsection{Input representation}
% \label{sec:method:input}


\subsection{Label Descriptions}
\label{sec:method:description}

A core component of our method is achieving \textcolor{red}{robust class latent representations}, making class encoding crucial. As a result, having additional information for each label is essential for our approach. In the datasets used for benchmarking, each relation is already accompanied by a concise and fixed description, which we refer to as the \textit{Raw description}. Although exploiting these descriptions during training RE model was investigated in \textbf{[CITE]} and achieved positive results, this approach was still limited as it depends on the limited 1-1 mapping between input embeddings and only one label description representation for each task. The poverty and restricted information of these kinds of texts not only hinder model optimization but also lead to instability of the corresponding learned representations.

To address this limitation, instead of using only an existing description for each class in each dataset, we take advantage of the power of pre-trained large language models (i.e, Gemini 1.5 \cite{team2023gemini, reid2024gemini}) to generate $K$ detailed, diverse and illustrative descriptions. In particular, when training each input sample, the respective raw description will be fed into \textit{the prompt}, serving as \textcolor{red}{\textit{"an expert in the loop"} to guide the LLM}. Our prompt template is depicted in Figure \ref{fig:tnse1}, with the corresponding output sample included in Appendix \ref{apdx:prompt_template}.

\begin{figure}[t!]
	\centering
	\includegraphics[width=\linewidth]{imgs/prompt-new-4.pdf}
	\caption{Prompt to generate label description.}
	\label{fig:tnse1}
\end{figure}


By exploiting LLMs in this way, we have achieved the retrieval of diverse and meaningful information for each training sample, thereby making the model generalize better, mitigating more efficiently in the challenging setting of FCRE.

% \subsection{Representation Learning}
% \label{sec:bg:replearning}

% In conventional Relation Extraction scenarios, a basic framework employing BERT, followed by a classification MLP, is often used to directly learn the mapping from the input space to the label space using Cross Entropy Loss. However, this approach proves inadequate in data-scarce settings \cite{snell2017prototypical}. Consequently, contrastive learning emerges as a more suitable approach, as it can directly influence the latent space and better capture the inherent distinctions between samples from different classes. To enrich the semantic information drawn from both the samples and the generated label descriptions, we design an objective function comprising four key loss components.


% % main components: $\mathcal{L}_{RE}$ to force relation embeddings..., and $\mathcal{L}_{Retrieval}$ to facilitate...
% % $$ \mathcal{L} = \mathcal{L}_{RE} + \mathcal{L}_{Retrieval}$$ where $\mathcal{L}_{RE}$ force relation embeddings..., and $\mathcal{L}_{Retrieval}$ facilitate ... 

% % \subsubsection{Relation extraction loss $\mathcal{L}_{RE}$}

% \paragraph{Supervised Contrastive Loss.}
% To enhance the model's discriminative capability, we employ the Supervised Contrastive Loss (SCL). This loss function is specifically designed to bring positive pairs of samples, which share the same class label, closer together in the latent space. Simultaneously, it pushes negative pairs, belonging to different classes, further apart. Let $\bm{z}_x$ represent the hidden vector output of sample ${x}$, the positive pairs $(\bm{z}_x, \bm{z}_p)$ are those who share a class, while the negative pairs $(\bm{z}_x, \bm{z}_n)$ correspond to different labels. The SCL is computed as follows:
% \begin{gather}
% \mathcal{L}_{\textrm{SC}}(x) = - \sum_{{p} \in P({x})} \log \frac{
%     f(\bm{z}_x, \bm{z}_p)
% }
% {Z_\textrm{SC}({x})}, \\
% Z_\textrm{SC}({x}) = \sum_{{p} \in P({x})} f(\bm{z}_x, \bm{z}_p) \  + \sum_{{n} \in N({x})} f(\bm{z}_x, \bm{z}_n), 
% \end{gather}
% where $f(\mathbf{x}, \mathbf{y}) \coloneqq \exp\left(\frac{\gamma(\mathbf{x}, \mathbf{y})}{\tau}\right)$, $\gamma(\cdot, \cdot)$ denotes the cosine similarity function, and $\tau$ is the temperature scaling hyperparameter. $P({x})$ and $N({x})$ denote the sets of positive and negative samples with respect to sample ${x}$, respectively.

% \paragraph{Hard Soft Margin Triplet Loss.}
% To achieve a balance between flexibility and discrimination, the Hard Soft Margin Triplet Loss (HSMT) integrates both hard and soft margin triplet loss concepts. This loss function is designed to maximize the separation between the most challenging positive and negative samples, while preserving a soft margin for improved flexibility. Formally, the loss is defined as:
% \begin{multline}
% \mathcal{L}_{\textrm{ST}}({x}) = - \log \bigg(1 \ +  
%     \max_{{p} \in P(\bm{x})} e^{\xi(\bm{z}_x, \bm{z}_p)} \\
%     - \min_{{n} \in N({x})} e^{ \xi(\bm{z}_x, \bm{z}_n)}
% \bigg),
% \end{multline}
% where $\xi(\cdot, \cdot)$ denotes the Euclidean distance function. The objective of this loss is to ensure that the hardest positive sample is as distant as possible from the hardest negative sample, thereby enforcing a flexible yet effective margin.


\subsection{Description Retrieval}
\label{sec:method:retrieval}

To encourage the knowledge of the retrieved descriptions to participate and effectively support the representation learning of input embeddings, we proposed exploiting the following objective function:
\begin{equation}
    \mathcal{L}_{Retrieval} = \beta_{HM}\cdot \mathcal{L}_{HM} + \beta_{MI}\cdot\mathcal{L}_{MI},
\end{equation}
where $\mathcal{L}_{HM}$ is \textit{Hard Margin loss}, $\mathcal{L}_{MI}$ is \textit{Mutual Information loss}, and $\beta_{HM},  \beta_{MI}$ are corresponding hyper-parameters. These two loss functions have symmetrical and mutually supportive roles, which are described in detail in what follows.  


\paragraph{Description-centered Alignment - DCA (Hard margin loss :vv)}

% \begin{align}
% \mathcal{L}_{\mathrm{MI}}(i) = - \log \frac{ \sum_{p \in P(i)} 
%     \exp \left(\frac{\gamma(\bm{z_p}, \bm{d_i})}{\tau}\right)
% }{
%     Z_{MI}(i)
% }
% % \exp \left(\frac{\gamma(\bm{z_i}, \bm{d_i})}{\tau}\right) 
% %     + \sum_{n \in N(i)} \exp \left(\frac{\gamma(\bm{z_n}, \bm{d_i})}{\tau}\right)
% \end{align}

% $$
% Z_{MI}(i) = {\sum_{p \in P(i)} \! \exp \left( \frac{\gamma(\bm{d_i}, \bm{z_p})}{\tau} \right) 
%   \!+\! \sum_{n \in N(i)} \! \exp \left(\frac{\gamma(\bm{d_i}, \bm{z_n})}{\tau} \right)} 
% $$

% The Hard Margin (HM) Loss focuses on maximizing the margin between hard positive and hard negative samples. Hard positive samples are those that are difficult to distinguish from the negative samples, and hard negative samples are those that are close to the positive samples in the latent space. The HM loss is defined as:

leverages each label description to refine the model's ability to distinguish between hard positive and hard negative pairs. Given a sample $\bm{x}$, one of the representation vectors of its corresponding retrieved descriptions is $\bm{d}^i_x$; $\bm{z}_p$ and $\bm{z}_n$ representing the hidden vectors of its positive and negative samples respectively. Then the loss function is formulated to maximize the similarity between $\bm{d}^i_x$ and the corresponding positive embeddings while pushing away the negative ones:
\begin{align}
% \begin{aligned}
    \mathcal{L}_{\textrm{HM}}(x) = &\sum_{p \in P_\textrm{H}(x)} (1 - \gamma(\bm{d}_x, \bm{z}_p))^2 \\
    &+ \sum_{n \in N_\textrm{H}(x)} max(0, m - 1 + \gamma(\bm{d}_x, \bm{z}_n) )^2,
% \end{aligned}
\end{align}
where $m$ is a margin parameter, $P_\textrm{H}(x)$ and $N_\textrm{H}(x)$ represent the sets of hard positive and hard negative samples, respectively. They are determined by comparing the similarity between $\bm{d}_x$ and both positive and negative pairs, specifically focusing on the most challenging pairs where the similarity to negative samples is close to or greater than that of positive samples, defined as follows:
\begin{align}
    \begin{aligned}
    P_\textrm{H}(x) = \{&p \in P(x) | 1 - \gamma(\bm{d}_x, \bm{z}_p) \\
    &> min_{n \in N(x)}(1 - \gamma(\bm{d}_x, \bm{z}_n)) \}
    \end{aligned}, \\
    \begin{aligned}
    N_\textrm{H}(x) = \{&n \in N(x) | 1 - \gamma(\bm{d_x}, \bm{z}_n) \\
    &< max_{p \in P(x)}(1 - \gamma(\bm{d}_x, \bm{z}_p)) \}.
    \end{aligned}
\end{align}

By utilizing the label description vector $\bm{d_x}$, the Hard Margin Loss effectively sharpens the model's decision boundary, reducing the risk of confusion between similar classes and improving overall performance in few-shot learning scenarios. The loss penalizes the model more heavily for misclassifications involving these hard samples, ensuring that the model pays particular attention to the most difficult cases, thereby enhancing its discriminative power.

\paragraph{Relation-centered constraint (Mutual Information Loss)}

The Mutual Information (MI) Loss is designed to maximize the mutual information between the input sample's hidden representation and its corresponding label description, promoting a more informative alignment between them. Let $\bm{d}_x$ represent the hidden vector corresponding to the label description of sample $\bm{x}$, and $\bm{d}_n$ the hidden vector of other label descriptions. According to \citet{DBLP:journals/corr/abs-1807-03748}, the Mutual Information $MI(x)$ between the input embedding $\bm{z}_x$ and its corresponding label description follows the following inequation:
\begin{equation}
    MI \geq \log B + \textnormal{InfoNCE} (\{ x_i\}_{i=1}^B; h),
\end{equation}
where we have defined:
\begin{gather}
\textnormal{InfoNCE} (\{ x_i\}_{i=1}^B; h) =
\frac{1}{B}\sum_{i=1}^B \log \frac{h(\bm{z_i}, \bm{d_i})}{\sum_{j=1}^B h(\bm{z_i}, \bm{d_j})}, \\
h(\bm{z}_x, \bm{d}_j) = \exp \frac{\bm{z}_x^TW\bm{d}_x}{\tau}
\end{gather}
where $\tau$ is the temperature, $B$ is mini-batch size and $W$ is a trainable parameter. Finally, the MI loss function in our implementation is: 
% \begin{equation}
%     \mathcal{L}_{MI} = -\sum_{(x_i , y_i) \in D_{train}^{k}}\textnormal{InfoNCE} (\{x_i\}_{i=1}^B; h)
% \end{equation}
\begin{align}
\mathcal{L}_{\textrm{MI}}(x) = - \log \frac{
    h(\bm{z}_x, \bm{d}_x)
}{
    h(\bm{z}_x, \bm{d}_x)
    + \sum_{n \in N(x)} h(\bm{z}_x, \bm{d}_n)
}
\end{align}

This loss ensures that the representation of the input sample is strongly associated with its corresponding label, while reducing its association with incorrect labels, thereby enhancing the discriminative power of the model.


\paragraph{Joint Training Objective Function.}
The final model is trained using a combination of the aforementioned loss functions, weighted by their respective coefficients:

\begin{align}
\begin{aligned}
\mathcal{L}(x) = &\beta_\textrm{SC} \cdot \mathcal{L}_{\textrm{SC}}(x) + \beta_\textrm{ST} \cdot \mathcal{L}_{\textrm{ST}}(x) \\
&+ \beta_\textrm{HM} \cdot \mathcal{L}_{\textrm{HM}}(x) + \beta_\textrm{MI} \cdot \mathcal{L}_{\textrm{MI}}(x)
\end{aligned}
\end{align}
where $\beta_\textrm{SC}$, $\beta_\textrm{ST}$, $\beta_\textrm{HM}$, and $\beta_\textrm{MI}$ are hyperparameters that balance the contribution of each loss term. This joint objective enables the model to leverage the strengths of each individual loss, facilitating robust and effective learning in Few-Shot Continual Relation Extraction tasks.


\subsection{Training Procedure}
\label{subsec:Framework}



% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\textwidth]{imgs/architecture.pdf}
%     \caption{ Our Framework.}
%     \label{fig:framework} 
%     \vspace{-.2cm}
% \end{figure}

\begin{figure}[t]
    \centering
    \hspace{-0.5cm} % Adjust the value as needed
    \includegraphics[width=0.5\textwidth]{imgs/architecture.pdf}
    \caption{Our Framework.}
    \label{fig:framework} 
    % \vspace{-.2cm}
\end{figure}

\begin{figure*}[t]
    \centering
    \hspace{-0.5cm} % Adjust the value as needed
    \includegraphics[width=1.\textwidth]{imgs/change_backbone.pdf}
    \caption{Adapting LLM2Vec for ours architecture}
    \label{fig:change_backbone} 
    % \vspace{-.2cm}
\end{figure*}


Algorithm \ref{alg:Framework} shows the end-to-end training for task $T_j$, with the model $\Phi_{j-1}$ previously trained. Following the memory-based methods for continual learning, we use a memory $\tilde{M}_{j-1}$ to preserve a few samples in all previous tasks $\{T_1,\dots,T_{j-1}\}$ and a relation description set $\tilde{K}_{j-1}$ to store the descriptions of all previous relations.

\begin{enumerate}
    \item \textbf{Initialization} (Line 1--2). 
    The current model $\Phi_j$ inherits the parameters of $\Phi_{j-1}$. We initialize $\Phi_j$ and update the relation description set $\tilde{K}_j$ by incorporating new relation descriptions from $K_j$.
    
    \item \textbf{Training the Current Task} (Line 3). 
    We adapt $\Phi_j$ on $D_j$ to learn the knowledge of new relations in $T_j$.
    
    \item \textbf{Memory Update} (Lines 4--8). 
    We initialize the memory $\tilde{M}_j$ from $\tilde{M}_{j-1}$. 
    % Inspired by \cite{han2020continual,cui2021refining},
    We select $L$ typical samples from $D_j$ for every relation $r \in R_j$, which constitute the memory $M_r$. The overall memory for all observed relations until now is $\tilde{M}_j = \tilde{M}_{j-1} \cup M_j$. The relation set is also updated as $\tilde{R}_j = \tilde{R}_{j-1} \cup R_j$.
    
    \item \textbf{Prototype Generation} (Line 9). 
    We generate a prototype set $\tilde{P}_j$ based on the updated memory $\tilde{M}_j$.
    
    % \item \textbf{Data Augmentation} (Line 10). 
    % Inspired by \textbf{CITE CPL}, to cope with the scarcity of samples, we generate an augmented dataset $D_j^*$ using ChatGPT, enhancing the training data with more variations.
    
    \item \textbf{Memory Training} (Line 10). 
    We update $\Phi_j$ by training on the augmented memory set $\tilde{M}_j^*$. This step helps in preserving the prior knowledge for identifying relations in previous tasks.
\end{enumerate}

We detail the procedure in the subsections below.


% Example
% \begin{algorithm}[ht]
% \caption{Adaptive Unified Gradient Descent for CRE} \label{alg:augd}
% \textbf{Input}: Model parameters $\bm{\theta}$ and differentiable loss functions $L_d$ and $L_{re}$\\
% \textbf{Parameter}: Learning rate $\eta$\\
% \textbf{Output}: Updated parameter $\bm{\theta}^{*}$
% \begin{algorithmic}[1]
% % \For{each task $t$}
% \FOR{each $t \in [d, re]$}
% \STATE Compute gradient $\bm{g}_t := \nabla_{\bm{\theta}} L_t(\bm{\theta})$
% \STATE Compute gradient unit vector $\bm{u}_t := \bm{g}_t / ||\bm{g}_t||$
% \ENDFOR
% \STATE Calculate gradient differences $\bm{D}^\top := \ \bigr[\bm{g}_{d}^\top - \bm{g}_{re}^\top\bigr]$.
% \STATE Calculate magnitude-scaled gradient unit differences:
% \begin{equation*}
%     \bm{U}^\top := \ \left[||\bm{g}_{re}||\bm{u}_{d}^\top - ||\bm{g}_{d}||\bm{u}_{re}^\top\right].
% \end{equation*}
% \STATE Calculate scalar coefficients for the objectives:
% \begin{align*}
% [\alpha_{re}] &= \bm{g}_{d}\bm{U}^\top(\bm{D}\bm{U^\top})^{-1}, \\
% \alpha_{d} &= 1 - \alpha_{re}.
% \end{align*}
% \STATE Update model parameter:
% \begin{equation*}
% \bm{\theta}^{*} = \bm{\theta} - \eta \sum_{i \in \{d, re\}} \alpha_{i}\bm{g}_{i}
% \end{equation*}
% \end{algorithmic}
% \end{algorithm}
% End example


\begin{algorithm}[ht]
\caption{Training procedure for $T_j$}
\label{alg:Framework}
\textbf{Input}: $\Phi_{j-1}, \tilde{R}_{j-1}, \tilde{M}_{j-1},\tilde{K}_{j-1}, D_j, R_j, K_j$. \\
\textbf{Output}: $\Phi_j, \tilde{M}_j, \tilde{K}_j$.
\begin{algorithmic}[1]
\STATE Initialize $\Phi_j$ from $\Phi_{j-1}$ 
\STATE $\tilde{K}_j \leftarrow \tilde{K}_{j-1} \cup K_j$
\STATE Update $\Phi_j$ by L on $D_j$ (train current task); 
\STATE $\tilde{M}_j \leftarrow \tilde{M}_{j-1}$
\FOR{each $r \in R_j$} 
    \STATE pick $L$ samples in $D_j$ and add them into $\tilde{M}_j$
\ENDFOR
\STATE $\tilde{R}_j \leftarrow \tilde{R}_{j-1} \cup R_j$\;
\STATE Generate prototype set $\tilde{P}_j$ based on $\tilde{M}_j$\;
 % \STATE Generate augmented dataset $D_j^*$ using ChatGPT\; 
\STATE Update $\Phi_j$ by $\mathcal{L}$ on $\tilde{M}_j$ and $D_j^*$ (train memory) 
\end{algorithmic}
\end{algorithm}

% \subsection{Reciprocal Rank Fusion
% Prediction}

% \begin{align}
% \text{RRF}(d) &= \sum_{i=1}^{n} \frac{1}{k + r_i(d)}
% \end{align}

% Where $n$ is the number of rankings being fused, $r_i(d)$ is the rank of document $d$ in the $i$-th ranking, $k$ is a constant.
% We leverage both the prototype and description to get the final fusion ranking. The first ranking is get by the euclid distance between the input and each prototype. The second ranking is get bt the cosine distance between the 

\subsection{Relation Prediction via Reciprocal Rank Fusion} \label{secrelationpre}

Building on the traditional Nearest-Class-Mean (NCM) approach \cite{ma-etal-2024-making}, our method enhances relation prediction by incorporating a retrieval mechanism based on reciprocal rank fusion. While the NCM classifier predicts relations by minimizing the Euclidean distance between the test sample $\bm{x}$ and the class prototypes derived from historical memory $\hat{\mathcal{M}}^n$, our approach augments this with the integration of cosine similarity measures, leveraging relation descriptions generated by a Large Language Model (LLM).

Given a sample $\bm{x}$ with hidden representation z and the set of relation prototypes ${p_r}_{r=1}^n$, we first calculate the NCM score for each prototype $p_r$:
% \begin{align}
% &p_r = \frac{1}{L} \sum_{i=0}^{L} \bm{E} \left(\bm{\hat{x}}_i^r\right), \notag \
% &\text{NCM_score}(r) = -{\left| \bm{E}\left(\bm{x}\right) - p_r\right|}_2
% \end{align}
\begin{align}
&p_r = \frac{1}{L} \sum_{i=1}^{L} \bm{E} \left(\bm{\hat{x}}_i^r\right), \notag \\
&\text{NCM}(x,r) = -{\left\| \bm{z} - p_r \right\|}_2
\end{align}


Simultaneously, we compute the cosine similarity between the hidden representation x and each relation description vector $\bm{d}_r$ generated by the LLM: $\gamma(\bm{z}, \bm{d_r})$


To robustly predict the relation, we then fuse the NCM and cosine similarity scores using a reciprocal rank fusion (RRF) strategy. The final prediction score for each relation $r$ is given by:

% \begin{align}
% &\text{RRF_score}(r) = \frac{1}{k + \text{rank}(\text{NCM_score}(r))} + \frac{1}{k + \text{rank}(\text{Cosine_score}(r))}
% \end{align}
% \begin{align}
% \text{RRF\_score}(r) = \frac{1}{k + \text{rank}\left(\text{NCM\_score}(x,r)\right)} + \frac{1}{k + \text{rank}(\text{\gamma(\bm{z}, \bm{d_r})})}
% \end{align}

\begin{align}
\begin{aligned}
\textrm{RRF}(r) = &\frac{1}{k + \text{rank}\left(\text{NCM}(x, r)\right)} + \frac{1}{k + \text{rank}\left(\gamma(\bm{z}, \bm{d}_r)\right)}
\end{aligned}
\end{align}


where $\text{rank}(\cdot)$ represents the rank position of the score among all relations, and $k$ is a small constant to avoid division by zero.

Finally, the relation label $y^*$ is predicted as the one corresponding to the highest RRF score:

% \begin{align}
% y^* = \underset{r=1, \ldots, n}{\operatorname{argmax}} , \text{RRF_score}(r)
% \end{align}

\begin{align}
y^* = \underset{r=1, \ldots, n}{\operatorname{argmax}} \, \text{RRF\_score}(r)
\end{align}



This fusion approach effectively balances the strengths of both NCM-based proximity and description-based semantic similarity, resulting in a more accurate and robust prediction across sequential tasks.




==> sections/aaai-checklist.tex <==
\begin{enumerate}

\item \textbf{This paper}:
    \item[] \textbf{Question:} Includes a conceptual outline and/or pseudocode description of AI methods introduced
    \item[] Answer: [YES]
    
    \item[] \textbf{Question:} Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)
    Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no)
    \item[] Answer: [YES]
    
\item \textbf{Does this paper make theoretical contributions?}
[NO]

\item \textbf{Does this paper rely on one or more datasets?}
[YES]

    \item[] \textbf{Question:} A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)
    \item[] Answer: [NO]. We would like to include the reason here: we follow the previous baselines in terms of benchmarking datasets, in order to conduct fair comparisons.
    
    \item[] \textbf{Question:} All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)
    \item[] Answer: [N/A]
    
    \item[] \textbf{Question:} All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
    \item[] Answer: [N/A]
    
    \item[] \textbf{Question:} All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations. (yes/no/NA)
    \item[] Answer: [YES]
    
    \item[] \textbf{Question:} All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available. (yes/partial/no/NA)
    \item[] Answer: [YES]
    
    \item[] \textbf{Question:} All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)
    \item[] Answer: [N/A]

\item \textbf{Does this paper include computational experiments?}
[YES]

    \item[] \textbf{Question:} Any code required for pre-processing data is included in the appendix. (yes/partial/no).
    \item[] Answer: [YES]. The source code for our experiments, along with detailed specifications for all external libraries utilized, has been submitted via the AAAI submission system. This provision ensures that researchers attempting to replicate our findings have comprehensive access to the necessary code base and dependencies.

    \item[] \textbf{Question:} All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)
    \item[] Answer: [YES]
    
    \item[] \textbf{Question:} All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)
    \item[] Answer: [YES]
     
    \item[] \textbf{Question:} All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)
    \item[] Answer: [YES]
    
    \item[] \textbf{Question:} If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)
    \item[] Answer: [YES]
    
    \item[] \textbf{Question:} This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)
    \item[] Answer: [YES]. This information is included in the Supplementary Materials accompanying the main PDF. We would like to specify here once more: Our BERT-based experiments were conducted on an NVIDIA RTX 3090 GPU with 24GB of memory. For experiments with the LLM2Vec backbone, we utilized an NVIDIA A100 GPU with 80GB of VRAM. The operating system used across all experiments was Ubuntu Server 18.04.3 LTS.
    
    \item[] \textbf{Question:} This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)
    \item[] Answer: [YES]. Evaluation metrics are described in the Supplementary Materials accompanying the main PDF.
    
    \item[] \textbf{Question:} This paper states the number of algorithm runs used to compute each reported result. (yes/no)
    \item[] Answer: [YES]. We run the algorithms 6 times. We include this information in the Supplementary Materials accompanying the main PDF.
    
    \item[] \textbf{Question:} Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)
    \item[] Answer: [YES]
    
    \item[] \textbf{Question:} The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)
    \item[] Answer: [NO]
    
    \item[] \textbf{Question:} This paper lists all final (hyper-)parameters used for each model/algorithm in the paper's experiments. (yes/partial/no/NA)
    \item[] Answer: [YES]
    
    \item[] \textbf{Question:} This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)
    \item[] Answer: [YES]. We include this information in the Supplementary Materials accompanying the main PDF.
    
\end{enumerate}

% This paper:
% \begin{itemize}
%     \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\textbf{\underline{yes}}/partial/no/NA)
%     \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\textbf{\underline{yes}}/no)
%     \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\textbf{\underline{yes}}/no)
% \end{itemize}

% \noindent
% Does this paper make theoretical contributions? (yes/\textbf{\underline{no}})

% \noindent
% Does this paper rely on one or more datasets? (\textbf{\underline{yes}}/no)
% \begin{itemize}
%     \item A motivation is given for why the experiments are conducted on the selected datasets (\textbf{\underline{yes}}/partial/no/NA)
%     \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/\textbf{\underline{NA}}).
%     We do not introduce novel datasets in this study.
%     \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/\textbf{\underline{NA}}).
%     We do not introduce novel datasets in this study.
%     \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\textbf{\underline{yes}}/no/NA)
%     \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\textbf{\underline{yes}}/partial/no/NA)
%     \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/\textbf{\underline{NA}}).
%     We do not use datasets that are not publicly available.
% \end{itemize}

% \noindent
% Does this paper include computational experiments? (\textbf{\underline{yes}}/no)
% \begin{itemize}
%     \item Any code required for pre-processing data is included in the appendix. (\textbf{\underline{yes}}/partial/no).
%     \item All source code required for conducting and analyzing the experiments is included in a code appendix. (\textbf{\underline{yes}}/partial/no)
%     \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\textbf{\underline{yes}}/partial/no)
%     \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\textbf{\underline{yes}}/partial/no)
%     \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\textbf{\underline{yes}}/partial/no/NA)
%     \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\textbf{\underline{yes}}/partial/no)
%     \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\textbf{\underline{yes}}/partial/no)
%     \item This paper states the number of algorithm runs used to compute each reported result. (\textbf{\underline{yes}}/no)
%     \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\textbf{\underline{yes}}/no)
%     \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/\textbf{\underline{no}})
%     \item This paper lists all final (hyper-)parameters used for each model or algorithm in the paper’s experiments. 
%     (\textbf{\underline{yes}}/partial/no/NA)
%     \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\textbf{\underline{yes}}/partial/no/NA)
%     \item \textbf{Source Code and Dependencies}: The source code for our experiments, along with detailed specifications for all external libraries utilized, has been submitted via the AAAI Rolling Review submission system. This provision ensures that researchers attempting to replicate our findings have comprehensive access to the necessary codebase and dependencies.
%     \item \textbf{Computing Infrastructure}: Our experiments involving a BERT-based model were conducted on an NVIDIA RTX 3090 GPU with 24GB of memory. For training the LLM2vec backbone, we utilized an NVIDIA A100 GPU with 80GB of VRAM. The operating system used across all experiments was Ubuntu Server 18.04.3 LTS.

% \end{itemize}

% \begin{itemize}
% \item \textbf{Source Code and Dependencies}: The source code for our experiments, along with detailed specifications for all external libraries utilized, has been submitted via the AAAI Rolling Review submission system. This provision ensures that researchers attempting to replicate our findings have comprehensive access to the necessary codebase and dependencies.
% \item \textbf{Computing Infrastructure}: Our experiments involving a BERT-based model were conducted on an NVIDIA RTX 3090 GPU with 24GB of memory. For training the LLM2vec backbone, we utilized an NVIDIA A100 GPU with 80GB of VRAM. The operating system used across all experiments was Ubuntu Server 18.04.3 LTS.
% \end{itemize}

==> sections/relatedwork.tex <==
\paragraph{Continual Learning (CL)}is a learning scenario that requires models to continually acquire new knowledge from a sequence of tasks while preventing the loss of previously learned information. The main challenge in CL is \textit{catastrophic forgetting} \citep{DBLP:conf/nips/French93}. To address this problem, memory-based approaches prove to be effective methods for both machine learning \citep{DBLP:conf/cvpr/RebuffiKSL17, DBLP:conf/nips/ShinLKK17} and NLP problems \citep{wang-etal-2019-sentence, han-etal-2020-continual}. In particular, models need to save a few representative samples from the current task in a memory buffer and replay these samples when learning new tasks to review old knowledge. 
% Current CL approaches are basically categorized into three types: 1) regularization methods \textbf{(Li and Hoiem, 2017; Ritter et al., 2018)}, which impose additional constraints to control updating of parameters, aiding the retention of older knowledge; 2) dynamic architecture methods \textbf{(Fernando et al., 2017; Mallya et al., 2018)}, which dynamically expand the model's architecture to accommodate new knowledge as new tasks arise; and 3) memory-based methods (Rebuffi et al., 2017; Shin et al., 2017), which save a few representative samples from the current task in memory and replay these samples when learning new tasks to review old knowledge. 
% Among these, memory-based methods are the most effective for NLP tasks \textbf{(Wang et al., 2019; Han et al., 2020)}. 

\paragraph{Fewshot Continual Relation Extraction} is a challenging scenario, which was introduced by \citep{DBLP:conf/acl/QinJ22} for Relation Extraction problems.  This challenge arises due to the limited availability of data for new tasks, coupled with the high cost and time involved in obtaining high-quality data. Recent work like \citet{DBLP:conf/acl/WangWH23, DBLP:conf/acl/ChenWS23, DBLP:conf/coling/MaHL024} propose memory-based solutions, which suggest imposing objective functions on the embedding space and classification head. Specifically, \citet{DBLP:conf/acl/WangWH23} employs serial objective functions based on contrastive and distillation,  \citet{DBLP:conf/acl/QinJ22} leverage extra training data from unlabeled text, and \citet{DBLP:conf/acl/ChenWS23} proposes a consistent prototype learning strategy to help the model distinguish between different relation representations, thus enhancing representation learning efficiency. 

% However, in these methods, eliminating the pre-trained LM head and training a new classifier still leads to overfitting and forgetting due to limited data, as it emphasizes discriminative features only. To address this problem, we propose a novel approach that leverages LM heads, which are often overlooked in pre-trained models for downstream tasks. Our method not only helps preserve prior knowledge from the backbone but also supports the training of the main classifier, thereby further reducing both catastrophic forgetting and overfitting.
% and significantly enhancing the model's performance, 


% Our approach also employs a memory-based strategy, but we focus more on optimizing the use of Pre-trained Language Models (PLMs) to address CFRE.
